Learning and Testing Latent-Tree Ising Models Efficiently

We provide time- and sample-efficient algorithms for learning and testing latent-tree Ising models, i.e. Ising models that may only be observed at their leaf nodes. On the learning side, we obtain efficient algorithms for learning a tree-structured Ising model whose leaf node distribution is close in Total Variation Distance, improving on the results of prior work. On the testing side, we provide an efficient algorithm with fewer samples for testing whether two latent-tree Ising models have leaf-node distributions that are close or far in Total Variation distance. We obtain our algorithms by showing novel localization results for the total variation distance between the leaf-node distributions of tree-structured Ising models, in terms of their marginals on pairs of leaves.

==> drawings.tex <==
% \begin{figure}[htbp]
% \centering
% \input{figures/quartet-KLM}
% \caption{Quartet + KLM}
% \label{fig:quartet-KLM}
% \end{figure}

% \begin{figure}[htbp]
% \centering
% \input{figures/cherry-movement-trace-old}
% \caption{Cherry movement trace caption}
% \label{fig:cherry-movement-trace-old}
% \end{figure}

\begin{figure}[htbp]
\centering
\input{figures/cherry-movement-trace}
\caption{
The figure illustrates how we transform the phylogenetic tree from (a) to (g) by shifting subtrees to form cherries.
(b) -- (d) fixes the cherries $\{e,h\}$ (see blue edges).
(d) -- (e) fixes the parents of the cherries $\{a,b\}$ and $\{f,g\}$ (see orange edges).
(e) -- (f) fixes the parents of the cherries $\{c,d\}$ and $\{e,h\}$ (see red edges).}
\label{fig:cherry-movement-trace}
\end{figure}
 
\begin{figure}[htbp]
\centering
\input{figures/appendix6}
\caption{Appendix Fig 6}
\label{fig:appendix6}
\end{figure}

\begin{figure}[htbp]
\centering
\input{figures/appendix7}
\caption{Appendix Fig 7}
\label{fig:appendix7}
\end{figure}

\begin{figure}[htbp]
\centering
\input{figures/appendix8}
\caption{Appendix Fig 8}
\label{fig:appendix8}
\end{figure}

\begin{figure}[htbp]
\centering
\input{figures/appendix9}
\caption{Appendix Fig 9}
\label{fig:appendix9}
\end{figure}

\begin{figure}[htbp]
\centering
\input{figures/appendix10}
\caption{Appendix Fig 10}
\label{fig:appendix10}
\end{figure}

\begin{figure}[htbp]
\centering
\input{figures/appendix11}
\caption{Appendix Fig 11}
\label{fig:appendix11}
\end{figure}

\begin{figure}[htbp]
\centering
\input{figures/appendix12}
\caption{Appendix Fig 12}
\label{fig:appendix12}
\end{figure}

==> proof-sketch-older.tex <==
\section{Technical contributions- Proof Sketch - older}

\subsection{Technical Tools for Theorem REF}

The goal now is to compare the distribution of topology $T$ with correlations $\alpha$ and $\hat{T}$ with correlations $\hat{\alpha}$. We will again make use of the expression in Lemma~\ref{l:basic_extend}, but now we also need to be specific about what topology is used in this formula, since it is not fixed. Hence, we define 

$$
f_x^T(\alpha) := 2^{-n} \cdot \sum_{\stackrel{S \subseteq [n]}{|S| \text{ even}}}\alpha_S\prod_{i \in S} x_i
$$
Note that the way the topology $T$ influences the expression is via the coefficients $\alpha_S$ that are defined in Section~\ref{sec:closed-form}, yet we suppress the dependence of these coefficients on $T$ to avoid overloading the notation. 

Thus, our task becomes to bound $|f_x^T(\alpha) - f_x^{\hat{T}}(\hat{\alpha})|$. When the topology was fixed, we did so by substituting one by one the coordinates of $\alpha$ with the ones from $\hat{\alpha}$. We
will now follow a similar path, but
instead of substituting $\alpha$'s, we will substitute the topology. 
In other words, we find a sequence of topologies $T^1=T, T^2,\ldots,T^m = \hat{T}$ that interpolates between $T,\hat{T}$ in a way that $T^i,T^{i+1}$ only differ in a small part of the graph. This is important, because the goal is to bound $|f_x^{T^i}(\alpha) - f_x^{T^{i+1}}(\alpha)|$ and then apply triangle inequality. Notice that in this process we are not changing the vector $\alpha$. Thus, the intermediate expressions $f_x^{T^i}(\alpha)$ do not necessarily correspond to true probability distributions. We will show however that this is not important for bounding TV. 

We now describe in more detail the sequence of local moves from $T$ to $\hat{T}$. To do that, we first need to introduce some useful concepts, inspired by the phylogenetics literature. We essentially want to characterize how different $T$ and $\hat{T}$ can be, given that $\alpha,\hat{\alpha}$ are close to each other.

\begin{figure}[htbp]
\centering
\input{figures/quartet-possibilities}
\caption{The three possible topologies for a quartet. 
In Possibility 1, the path from $1$ to $2$ does not intersect the path from $3$ to $4$. Further, $\alpha_{12}\alpha_{34} \ge \alpha_{13}\alpha_{24} = \alpha_{14}\alpha_{23}$ (and similarly for Possibilities 2 and 3).}
\label{fig:quartet-possibilities}
\end{figure}

We will use the notion of a quartet of leaves: this is a collection of four leaves, which we denote by $1,2,3$ and $4$ in the discussion. These leaves can connect in the tree in three ways, as depicted in Figure~\ref{fig:quartet-possibilities}. There are three quantities that determine the true connection out of these three possibilities, and those quantities are $\alpha_{12}\alpha_{34}$, $\alpha_{13}\alpha_{24}$ and $\alpha_{14}\alpha_{23}$. The two smallest quantities are always equal, while the identity of the largest quantity determines the true topology. We would like to define a parameter that captures how sensitive is the quartet $(1,2,3,4)$ to changing $\alpha$. If this parameter is small, then a small change in $\alpha$ might incur a change in the tolopogy between these leaves and vice versa. 
For this purpose, define
\begin{align*}
\Delta_{ijkl} := \max(\alpha_{12}\alpha_{34}, \alpha_{13}\alpha_{24}, \alpha_{14}\alpha_{23}) - \min(\alpha_{12}\alpha_{34}, \alpha_{13}\alpha_{24}, \alpha_{14}\alpha_{23})
\end{align*}

We say that a quartet of leaves $i,j,k,l$ is an $\epsilon$-\emph{bad quartet} if and only if $\Delta_{ijkl} \leq \epsilon$. 
If a quartet is not a bad quartet, we say it is an $\epsilon$-\emph{good quartet}.  It is well known in the phylogenetics literature that for every quartet $i,j,k,l$ there are $3$ topologically distinct ways that these $4$ leaves are connected to each other, if we contract all the paths leading to other leaves in the tree. 
Depending on which of the $3$ ways we have, we say that the tree \emph{induces} a topology for a specific quartet. 
If two trees induce a different topology for a quartet, we say that the trees \emph{disagree} on that quartet, otherwise we say they \emph{agree}.
We know (folklore) that if two trees agree on all the quartets, then the two trees should be identical. 
Hence, the measure of dissimilarity between two trees that we will use is in how many quartets they disagree. 
Intuitively, if a quartet is bad, then we will not be able to distinguish which of the 3 possible topologies is the correct from samples. 
Indeed, it is easy to see that if $\alpha,\hat{\alpha}$ are $\epsilon$-close, then $\hat{T}$ and $T$ will only potentially disagree on $2\epsilon$-bad quartets. Hence, the goal of the sequence of local moves will be to gradually reduce the number of quartets where $T$ and $\hat{T}$ disagree, while guaranteeing that at every step only the topology of bad quartets changes. After finding such a sequence of moves, our goal will be to show that TV distance doesn't change much if the topology only changes for some bad quartets. 
Intuitively, the quartets are the analog of the pairwise distances for the fixed topology. While in the fixed topology case we substituted the pairwise distances one by one, here we will "substitute" all the quartets with the wrong topology one by one, until we reach $\hat{T}$.

Let us now describe the sequence of moves in a bit more detail. For more information, see Section REF. 
First, we define a pair of leaves to be a \emph{cherry} if they share their common neighbor (recall that a leaf has only one neighbor). In other words
We start
by identifying two leaves $i,j$ that are a cherry in $\hat{T}$ but are not a cherry in $T$ (what's a cherry?). Without loss of generality, we can assume that such a pair exists. We will describe later what happens if it does not. Since $i,j$ are not a cherry in $T$, there is a path $P_{ij}$ connecting them, which involves at least $2$ other nodes. Let $v_1 = i,v_2,\ldots, v_l = j$ with $l \geq 4$. Also, suppose that $i$ has a weaker connection than $j$ in $\hat{T}$, in the metric that induces $\hat{\alpha}$. We will start moving $i$ along the path $P_{ij}$ until it becomes a cherry with $j$. The different steps of this movement are shown in Figure~\ref{fig:ladder-movement}, where we can see with different colors the different positions of $i$. When this is done, we will find a new pair to make a cherry and so on. If $T$ and $\hat{T}$ agree on cherries, then we look at the parents of the cherries for new cherries. If this process ends without finding a cherry of $\hat{T}$ that is not a cherry of $T$, then $T$ and $\hat{T}$ are the same.


Let us focus on the first step of this process. This involves cutting $i$ from it's current place and pasting it in the middle of edge $(v_2,v_3)$, as shown in Figure~\ref{fig1}. This produces a tree $T^2$. We would like to argue that $|f_x^{T^1}(\alpha) - f_x^{T^2}(\alpha)|$ is small. To do that, we first prove the following lemma.

\begin{lemma}\label{l:lipschitz_quartet}
Let $i,j$ be a cherry in $\hat{T}$ but not in $T$ and let $T^2$ be the topology defined by procedure REF. Also, denote by $U$ the set of quartets where $T$ and $T^2$ disagree on. 
Then,
$$
\sum_{x \in \{-1,1\}^n} |f_x^T(\alpha) - f_x^{T^2}(\alpha)| \leq \sum_{(i,j,k,l)\in U} \Delta_{ijkl}
$$
\end{lemma}
Lemma~\ref{l:lipschitz_quartet} can be seen as an analog of Lemma~\ref{l:lipschitz}, but now instead of pairwise distances we have the quartets. It shows a type of Lipschitzness of $f_x^T$ when we change the topology of some of the quartets. The way to prove it is to notice that the difference $|f_x^T(\alpha) - f_x^{T^2}(\alpha)|$ can be factored into a sum of terms, each for a quartet in $U$. This term is the expression of a probability distribution on a topology that results when we remove all paths between leaves in that quartet from the tree. This is analogous to the property we observed about Lipschitzness w.r.t. a pairwise correlation in the fixed topology case.

Hence, if we apply Lemma~\ref{l:lipschitz_quartet} for the loss in TV in the first step of the sequence, we need to argue that $\Delta_{ijkl}$ is small for all $(i,j,k,l)\in U$. In other words, we need to argue that
all the quartets that change topology in one step are bad quartets. To give some intuition about this, let's observe what are the quartets that change topology in one step. As we can see in Figure~\ref{fig1}, quartet $\{(ik)(lm)\}$ becomes $\{(kl)(im)\}$ after the first step. Now, suppose it is a good quartet. Then, by definition of $\Delta$, we should have $\alpha_{ik}\alpha_{lm} - \alpha_{im}\alpha_{kl} = \Omega(\epsilon)$. This implies that
 $\hat\alpha_{ik}\hat\alpha_{lm} - \hat\alpha_{im}\hat\alpha_{kl} = \Omega(\epsilon)$. Since $i,j$ are a cherry in $\hat{T}$, we can replace $i$ with $j$ in any quartet involving the rest of the leaves (since $j$ has the stronger link) and this implies
 $\hat\alpha_{jk}\hat\alpha_{lm} - \hat\alpha_{jm}\hat\alpha_{kl} = \Omega(\epsilon)$. This finally means that  $\alpha_{jk}\alpha_{lm} - \alpha_{jm}\alpha_{kl} = \Omega(\epsilon)$. Now that is a contradiction, since it implies that the correct topology in $T$ is $\{(jk)(lm)\}$, while we can see that it is $\{(kl)(mj)\}$. 


After ensuring that $\Delta_{ijkl}$ is small, the natural next step would be to repeatedly apply Lemma~\ref{l:lipschitz_quartet} for each step of the sequence of trees and obtain a bound for $|f_x^T(\alpha) - f_x^{\hat{T}}(\alpha)|$, using triangle inequality. Unfortunately, we cannot apply Lemma~\ref{l:lipschitz_quartet} directly for each intermediate step in the sequence, because the expressions $f_x^{T^i}$ do not necessarily represent probability distributions anymore. This is a similar issue to the one we faced in proving Theorem REF. The way to overcome it is to again use a careful induction on the number of steps to argue that the Lipschitzness with respect to a quartet is still small at any intermediate point in the sequence (for details see Section REF).

The final step is to substitute $\alpha$ with $\hat{\alpha}$, which gives us error $|f_x^{\hat{T}}(\alpha) - f_x^{\hat{T}}(\hat{\alpha})|$. However, this error can be controlled, as the expressions come from the same topology $\hat{T}$. Hence, we can use the technique of Theorem REF to bound this quantity. This concludes the proof of Theorem REF. 


==> proof/changes.tex <==
\section{Changes from the original submission}

We note that while preparing the supplementary material and after a careful proofreading, we discovered that two of our theorems have slightly changed. First, our guarantee of Theorem~\ref{thm:alg} (unknown topology) has an improved sample complexity: $O(n^18 \log^3(n/\delta)/\epsilon^6)$ to $O(n^14 \log(n/\delta)/\epsilon^6)$. The second change is of Theorem~\ref{thm:probabilistic}. Here, the guarantee is 

==> tvbound_different_topo.tex <==
\section{Proof of Theorem~\ref{thm:probabilistic} 2.}
In this Section, we prove the following Theorem.
\vardis{maybe make the intro theorem restatable}

\begin{theorem}
Let $\hat{T},T^*$ denote the topologies of two trees with $n$ leaves, where each non-leaf node has degree $3$. Let $\hat{\alpha},\alpha^* \in [0,1]^{n \choose 2}$ denote vectors of pairwise distances that are induced by some tree metric on $\hat{T}$ and $T^*$, respectively. 
Also, let $\hat{mu}$ and $\mu^*$ be distributions over the leaves of $\hat{T}$ and $T^*$ when the pairwise 
\end{theorem}

we present an improved algorithm for estimating the distribution of leaves in TV distance when the topology of the underlying tree is unknown. At the core of the argument lies a bound on the total variation distance of two distributions of leaves with potentially different underlying topologies. To motivate the discussion, let's start with some definitions. As always, the true topology is denoted by $T$ and the vector of all the correct pairwise distances is $\alpha$. 

\begin{definition}
Let $i,j,k,l$ be a quartet of four leaves of $T$. We define 
$$
\Delta_{ijkl} := \max(\alpha_{12}\alpha_{34}, \alpha_{13}\alpha_{24}, \alpha_{14}\alpha_{23}) - \min(\alpha_{12}\alpha_{34}, \alpha_{13}\alpha_{24}, \alpha_{14}\alpha_{23})
$$
$$
\hat\Delta_{ijkl} := \max(\hat\alpha_{12}\hat\alpha_{34}, \hat\alpha_{13}\hat\alpha_{24}, \hat\alpha_{14}\hat\alpha_{23}) - \min(\hat\alpha_{12}\hat\alpha_{34}, \hat\alpha_{13}\hat\alpha_{24}, \hat\alpha_{14}\hat\alpha_{23})
$$
\end{definition}
\begin{definition}
Let $i,j,k,l$ be a quartet of four leaves of $T$. We say that this is an \emph{$\epsilon$-good quartet} if 
$$
\Delta_{ijkl} \geq \epsilon
$$
\end{definition}

A quartet of leaves that is not an $\epsilon$-good quartet is called an \emph{$\epsilon$-bad quartet}. 
Intuitively, if a quartet is good, then it is easy for an algorithm to distinguish which is the correct topology of these four leaves out of the three possibilities. If it is bad, then the topology is very close to being a star and so all three possibilities are roughly equivalent.
One thing to note is that our estimates $\hat{\alpha}$ imply that
$$
|\Delta_{ijkl} - \hat{\Delta}_{ijkl}| \leq \epsilon
$$
for all $i,j,k,l$. Hence, it does not really make a difference whether a quartet is good or bad in $T$ or in $\hat{T}$, since there is only an $\epsilon$-additive error. 


We now briefly describe the algorithm that we will use. We will not argue in detail about it's computational or statistical complexity, but instead focus on the quality of approximation that it gives in terms of TV distance. We will see that it is easy to argue about the sample complexity of the algorithm once we have everything else.

The algorithm works as follows: first it finds $\epsilon$-approximations for all the pairwise distances, and also classifies all quartets into $\epsilon$-good or $\epsilon$-bad. Then, it finds a topology $\hat{T}$ and estimates $\hat{\alpha}$ such that the following two properties hold
\begin{itemize}
    \item $|\alpha_{ij} - \hat{\alpha}_{ij}| \leq \epsilon$
    \item If a quartet is $\epsilon$-good for $T$ or $\hat{T}$, then this quartet will have the same topology in $T$ and $\hat{T}$. 
\end{itemize}

Our goal will be to prove that these properties are enough to guarantee that the estimated distribution is close enough to the true distribution. 
For this purpose, we will prove the following Theorem.

\begin{theorem}
Let $\hat{T}$ be the output of the algorithm with parameter $\epsilon/(2n^4)$.
Then,
$$
TV(P,\hat{P}) \leq  \epsilon
$$
\end{theorem}

The first step to the proof of the Theorem is the following Lemma, which showcases the main ideas needed in the proof.  

\begin{lemma}\label{l:cut_paste}
Let $\epsilon > 0$ and suppose we run the algorithm with accuracy $\epsilon/ n^4$. 
Suppose $i,j$ are two leaves that form a cherry in $\hat{T}$ but not in $T$. Let $u$ be their common parent in $\hat{T}$ and suppose that $\hat{\alpha}_{iu} < \hat{\alpha}_{ju}$. Let $\Bar{T}$ be the topology that results from $T$ if we cut leaf $i$ from it's place in $T$ (we also remove it's edge to the parent) and glue it so that it forms a cherry with $j$. 
Then
$$
\sum_{x \in \{-1,1\}^n} |f_x^T(\alpha) - f_x^{\Bar{T}}(\alpha)| \leq \frac{\epsilon}{n}
$$
\end{lemma}
\begin{proof}
Let $P(i,j) = v_1, \ldots, v_l $ be the path between leaves $i,j$ in $T$, meaning that $v_1 = i , v_l = j$. 
We will define a series of topologies, starting with $T^1 = T$. $T^2$ is defined by cutting leaf $i$ from it's current place and splitting edge $(v_3,v_4)$ into two edges $(v_3,w_2),(v_4,w_2)$ and adding an edge $(w_2,i)$. In general, for $k \leq l -2$, we define $T^k$ to be the topology obtained by $T$ by cutting leaf $i$ from it's original place, splitting edge $(v_{2 + i},v_{3 + i})$ into two edges $(v_{2+i}, w_k), (w_k, v_{3+i})$ and adding the edge $(w_k ,i)$. It is clear from the definition that 
$T^{l-2} = \Bar{T}$. Clearly, we do not have to define weights on each of these topologies, as we are only interested in the pairing that they induce for the various subsets of leaves. Using triangle inequality, we can write
\begin{equation}\label{eq:first_step}
\sum_{x \in \{-1,1\}^n} |f_x^T(\alpha) - f_x^{\Bar{T}}(\alpha)| \leq \sum_{k = 1}^{l-3} \sum_{x \in \{-1,1\}^n} |f_x^{T^{k+1}}(\alpha) - f_x^{T^k}(\alpha)|
\end{equation}
We will bound each term corresponding to some $k$ separately. Let $r_k$ be the number of quartets that will have different topology in $T^k$ and $T^{k+1}$.
Specifically, we are going to prove that for each $k$ 
$$
 \sum_{x \in \{-1,1\}^n} |f_x^{T^{k+1}}(\alpha) - f_x^{T^k}(\alpha)| \leq \frac{\epsilon r_k}{n^4}
$$
We will prove this inductively. Let's start with the case $k = 1$. We examine which terms in the expressions $f_x^{T^{2}}(\alpha), f_x^{T^{1}}(\alpha)$ are different.  First of all, since all internal nodes have degree $3$, each node $v_i$ of the path has a subtree $U_i$ hanging from it, except $v_1,v_l$. We will examine all even subsets of leaves in terms of which subtrees they intersect. First of all, if a subset of leaves does not contain $i$, then the splitting into pairs is not affected by the change in the topology, since the relative topology of the leaves other than $i$ remains the same. Hence, let $S$ be an even subset that contains $i$. Then $S_i := S\setminus\{i\}$ has odd cardinality. Notice that $S_i$ can be partitioned into the subsets $S_i \cap (U_2 \cup U_3)$ and $S_i \cap \lp(\cup_{j \geq 4} U_j\rp)$. 
There are two possibilities:
\begin{itemize}
    \item $|S_i \cap (U_2 \cup U_3)|$ is odd and $|S_i \cap \lp(\cup_{j \geq 4} U_j\rp)|$ is even. In that case, the leaves in $S_i \cap (U_2 \cup U_3)$ will be paired in the same way in $T^1,T^2$, except one leaf, which will be paired with $i$ in both topologies. The leaves in $S_i \cap \lp(\cup_{j \geq 4} U_j\rp)$ will
    be paired the same way in $T^1,T^2$. Hence, the term corresponding to subset $S$ will be the same in $T^1$ and $T^2$ in that case.
    \item $|S_i \cap (U_2 \cup U_3)|$ is even and $|S_i \cap \lp(\cup_{j \geq 4} U_j\rp)|$ is odd. In that case, there are two subcases:
    \begin{itemize} 
        \item $|S_i \cap U_2|, |S_i \cap U_3|$ are both even. In that case, leaves in $S_i \cap U_2$ will be paired the same way in $T^1,T^2$ and the same holds for $S_i \cap U_3$. The leaves in $S_i \cap \lp(\cup_{j \geq 4} U_j\rp)$ will be paired in the same way and one leaf will be left alone and will be paired with $i$ in both $T^1,T^2$. As a result,
        the term corresponding to $S$ will be the same in $T^1,T^2$. 
        \item $|S_i \cap U_2|, |S_i \cap U_3|$ are both odd. In that case, the leaves in $S_i \cap U_2$ will be paired the same way in both $T^1,T^2$, with one leaf $u_2 \in U_2$ left alone. Similarly for $S_i \cap U_3$ and one leaf $u_3 \in U_3$. For leaves in $S_i \cap \lp(\cup_{j \geq 4} U_j\rp)$, they will again be paired the same way, leaving one leaf $u_4 \in \cup_{j \geq 4} U_j$ alone. Now, in $T^1$, $i$ will be paired with $u_2$ and $u_3$ will be paired with $u_4$. However, in $T^2$ $i$ will be paired with $u_4$ and $u_2$ with $u_3$. 
    \end{itemize}
\end{itemize}
After this case analysis, it is clear that $S$ will have a different expression in $T^1,T^2$ if and only if $S$ is of the form
$$
S = \{i,u_2,u_3,u_4\}\cup S_2\cup S_3 \cup S_4
$$
with $S_2 \subseteq U_2, S_3 \subseteq U_3, S_4 \subseteq \cup_{j\geq 4} U_j$ and the extra constraint that $U_2$ lies on the subtreee that is disconnected from $i$ if we remove the path from $u_2$ to $i$ and similarly for $U_3,U_4$. This proves first of all that $r_1 = |U_2||U_3||\cup_{j \geq 4} U_j|$. Second, it proves that \vardis{up to constants}
\begin{align}\label{eq:quartet_split}
 \sum_{x \in \{-1,1\}^n} |f_x^{T^{k+1}}(\alpha) - f_x^{T^k}(\alpha)|  &= \lp|\sum_{x \in \{-1,1\}^n} \sum_{u_2 \in U_2, u_3 \in U_3, u_4 \in \cup_{j \geq 4}U_j} (\alpha_{iu_2}\alpha_{u_3u_4} - \alpha_{i u_4}\alpha_{u_2u_3}) x_i x_{u_2}x_{u_3}x_{u_4} P_{G\setminus \{i,u_2,u_3,u_4\}}(x) \rp|
\end{align}

where $P_{G\setminus \{i,u_2,u_3,u_4\}}(x)$ is the probability distribution of the rest of the leaves when the paths that belong to the quartet $i,u_2,u_3,u_4$ are removed. Notice that this topology will be the same regardless of whether we remove it from $T^1$ or $T^2$ and also that it is indeed a probability distribution. Now, the only thing we need to check in order to bound this quantity is that the quartet $i,u_2,u_3,u_4$ is bad. Suppose for contradiction that we have
$
\Delta_{iu_2u_3u_4} = \Omega(\epsilon/n^4)
$
\vardis{We will figure out the constants later}
Then, by the approximation guarantee of the algorithm
\begin{equation}\label{eq:posi}
\hat\Delta_{iu_2u_3u_4} = \Omega(\epsilon/n^4)
\end{equation}
We have chosen $i$ so that $\hat\alpha_{iu} < \hat{\alpha}_{ju}$ in the estimated model $\hat{T}$, so this implies that $j,u_2,u_3,u_4$ is also a good quartet, meaning
\begin{equation}\label{eq:posj}
\hat\Delta_{ju_2u_3u_4} = \Omega(\epsilon/n^4)
\end{equation}
Now, inequalities \eqref{eq:posi} and \eqref{eq:posj} give us a contradiction. The reason is that they suggest that both $i$ and $j$ are correctly positioned in $T$ relative to $u_2,u_3,u_4$ (correctly here means in terms of $\hat{T})$. But their relative positioning $i,j$ in $T$ is different and we know that they are siblings in $\hat{T}$, which means that
they should have the same positioning relative to any quartet. This leads us to a contradiction. This means that $iu_2u_3u_4$ is a bad quartet, hence $\Delta_{iu_2u_3u_4} = O(\epsilon/n^4)$. This implies that we did not violate any good quartets by changing from $T^1$ to $T^2$. Thus, equation \eqref{eq:quartet_split} implies
\begin{align*}
   \sum_{x \in \{-1,1\}^n} |f_x^{T^{k+1}}(\alpha) - f_x^{T^k}(\alpha)|  &= \lp|\sum_{u_2 \in U_2, u_3 \in U_3, u_4 \in \cup_{j \geq 4}U_j} \sum_{x \in \{-1,1\}^n} (\alpha_{iu_2}\alpha_{u_3u_4} - \alpha_{i u_4}\alpha_{u_2u_3}) x_i x_{u_2}x_{u_3}x_{u_4} P_{G\setminus \{i,u_2,u_3,u_4\}}(x) \rp|\\
 &\leq \sum_{u_2 \in U_2, u_3 \in U_3, u_4 \in \cup_{j \geq 4}U_j} \sum_{x \in \{-1,1\}^n} \Delta_{iu_2u_3u_4}  P_{G\setminus \{i,u_2,u_3,u_4\}}(x) \\
 &\leq \frac{\epsilon}{n^4} |U_2||U_3||\cup_{j \geq 4} U_j| = \frac{\epsilon r_1}{n^4}
\end{align*}

Hence, the base case of the induction is complete. Now, let us try to complete the induction. Suppose the statement holds for all $k < m$. We will prove it for $ k = m$. 
First of all, we examine which terms in the expressions $f_x^{T^{m+1}}(\alpha), f_x^{T^{m}}(\alpha)$ are different. It is not hard to see that similarly to the analysis for the base case, we have that a subset $S$ has different expression if and only if it can be written as
$$
S = \{i, u_2, u_3, u_4\} \cup S_2 \cup S_3 \cup S_4
$$
where $u_2 \in \cup_{j \leq m } U_j, u_3 \in U_{m+1}, u_4 \in \cup_{j \geq m+2}U_j$ and $|S_2|,|S_3|,|S_4|$ even any lying on the subtrees that result when removing the paths of the quartet $i,u_2,u_3,u_4$ from $T^m$. This shows that $r_m = |\cup_{j \leq m } U_j||U_{m+1}||\cup_{j \geq m+2}U_j|$. It also follows from this characterization that
the sets of quartets that change in each step of moving $i$ are disjoint from each other.
This means that
$$
\sum_m r_m \leq n^3
$$
since the total number of quartets that $i$ is involved in is $n^3$. Similar to the base case, we can write
\begin{align*}
 \sum_{x \in \{-1,1\}^n} |f_x^{T^{m+1}}(\alpha) - f_x^{T^m}(\alpha)|  &= \lp|\sum_{u_2 \in \cup_{j \leq m} U_j, u_3 \in U_{m+1}, u_4 \in \cup_{j \geq m+2}U_j} \sum_{x \in \{-1,1\}^n} (\alpha_{iu_2}\alpha_{u_3u_4} - \alpha_{i u_4}\alpha_{u_2u_3}) x_i x_{u_2}x_{u_3}x_{u_4} P_{T^m\setminus \{i,u_2,u_3,u_4\}}(x) \rp|
\end{align*}
Notice that $P_{T^m\setminus \{i,u_2,u_3,u_4\}}$ is still a true distribution over the remaining leaves, since $i$ is disconnected from the topology and the remaining topology is the correct one. Using the same argument as in the base case, we can prove that by moving $i$ one step, we do not violate any of the good quartets(otherwise $j$ would violate them as well). Hence, we conclude that
$$
 \sum_{x \in \{-1,1\}^n} |f_x^{T^{k+1}}(\alpha) - f_x^{T^k}(\alpha)| \leq 
 \frac{r_m \epsilon}{n^4}
$$
and the induction proof is complete. 
Now, from inequality \eqref{eq:first_step} we obtain
\begin{align*}
\sum_{x \in \{-1,1\}^n} |f_x^T(\alpha) - f_x^{\Bar{T}}(\alpha)| &\leq \sum_{k = 1}^{l-3} \sum_{x \in \{-1,1\}^n} |f_x^{T^{k+1}}(\alpha) - f_x^{T^k}(\alpha)|\\
&\leq \frac{\epsilon}{n^4} \sum_k r_k \leq \frac{\epsilon}{n}
\end{align*}



\end{proof}

We now move on with the proof of Theorem REF. The idea is to apply Lemma~\ref{l:cut_paste} repeatedly, starting from $T$. Each time we reconstruct some cherry of $\hat{T}$ or a generalized cherry(cherry of two internal nodes whose subtrees already agree with $\hat{T}$). It is easy to see that a total of $n$ of these operations suffice to move from $T$ to $\hat{T}$. The challenge is that in every intermediate step other than the first one, the lipschitzness will actually not correspond to a true probability distribution. Therefore, we have to use the technique that was developed in the previous Section for fixed topology. That way we can control the errors and show that if they are small enough, we still get a good bound on the TV distance. 

\begin{proof}
We will define a sequence of graphs $T_1,\ldots,T_{n-1}$ with $T_1 = T$ and $T_{n-1} = \hat{T}$. The general way of defining the sequence is as follows: 
at every step $i$, we maintain that some internal nodes of $T_i$ might have a subtree that has identical topology with the one in $\hat{T}$. We treat this subtree as nonexistent for the problem of selecting the next cherry. By pruning these subtrees, we are left with a tree $\Bar{T_i}$. Then, we 
pick two leaves $i,j$ that are cherries in $\hat{T}$ but not in $\Bar{T_i}$ (such a pair should exist, otherwise a larger subtree would have to be pruned). Suppose without loss of generality that $i$ has a weaker link than $j$ in $\hat{T}$ (the precise definition is similar to the one in Lemma~\ref{l:cut_paste}). 
Then, we define $T_{i+1}$ to be the tree that arises from $T_i$ if we cut $i$ from $T_i$ and glue it so that it becomes a cherry with $j$. During this process, any subtrees that are hanging from $i$
will also be transferred together with $i$. It is clear that $T_{i+1}$ is more similar to $\hat{T}$ than $T_i$ and after $n$ of these operations we will actually reach $\hat{T}$. The reason is that the total size of all the subtrees that agree with $\hat{T}$ increases by $1$. 
We will bound the error in each of these steps separately. Lastly, we will substitute $\alpha$ with $\hat{\alpha}$ using the argument we have for a fixed topology and this will conclude the proof.

In order to go from topology $T_i$ to $T_{i+1}$ we use a procedure similar to the one defined in Lemma~\ref{l:cut_paste}, by moving a leaf edge by edge until it reaches the correct spot. Hence, we have a sequence $\{T_i^j\}_{j = 1}^{l_i}$ with $T_i^1 = T_i, T_i^{l_i} = T_{i+1}$. Hence, for each step of the transformation, we can index it as $(i,j)$, if the current tree is $T_i^j$. 

Our argument will be an induction on the total number of quartets that have been altered since our transformation began. 
Clearly, when $i$ or $j$ increases, this number increases. We will prove that for any step $(i,j)$ in that process, if $K_{ij}$ is the total number of quartets that have been altered until that point in the transformation, we have

$$
\sum_{x \in \{-1,1\}^n} |f_x^T(\alpha) - f_x^{T_i^j}(\alpha)| \leq \frac{\epsilon K_{ij}}{n^4}
$$

The base case of the induction was  proved in Lemma~\ref{l:cut_paste}. Suppose it holds for all $(i',j')$ up until $(i,j)$. We will prove it for $(i,j)$. 
We have that
\begin{equation}\label{eq:Kij}
\sum_{x \in \{-1,1\}^n} |f_x^T(\alpha) - f_x^{T_i^j}(\alpha)| \leq 
\sum_{k <  i} \sum_{m \leq l_k}\sum_{x \in \{-1,1\}^n}  |f_x^{T_k^{m+1}}(\alpha) - f_x^{T_k^m}(\alpha)| + \sum_{m \leq j} \sum_{x \in \{-1,1\}^n}  |f_x^{T_i^{m+1}}(\alpha) - f_x^{T_i^m}(\alpha)|
\end{equation}
Let's pick some $k < i, m \leq l_k$. The case $k = i$ is identical. 
Let $u,v$ be the cherry picked at the step $k$ with $u$ moving towards $v$. 


We would like to bound each individual term of the sum similarly to the way we did it in Lemma~\ref{l:cut_paste}. However, the problem is that  the difference 
$|f_x^{T_k^{m+1}} (\alpha) - f_x^{T_k^m}(\alpha)|$ does not necessarily correspond to a probability distribution. The reason is that part of the topology of $T_k$ corresponds to $T$ and part of it to $\hat{T}$ (only at the first step this isn't true). Hence,
we need to handle these errors with extra care. First of all, for a given $m$, we know that the expressions $f_x^{T_k^{m+1}} (\alpha) , f_x^{T_k^{m}} (\alpha) $ differ only in terms that involve some quartet $i,u_2,u_3,u_4$, where $u_2,u_3,u_4$ are defined exactly as in Lemma~\ref{l:cut_paste}. Also, a similar argument shows that all these are bad quartets. This enables us to write
\begin{align*}
 \sum_{x \in \{-1,1\}^n} |f_x^{T_k^{m+1}}(\alpha) - f_x^{T_k^m}(\alpha)|  =\\
 =\sum_{x \in \{-1,1\}^n} \lp|\sum_{u_2 \in \cup_{j \leq m} U_j, u_3 \in U_{m+1}, u_4 \in \cup_{j \geq m+2}U_j}
 \sum_{x \in \{-1,1\}^n} (\alpha_{iu_2}\alpha_{u_3u_4} - \alpha_{i u_4}\alpha_{u_2u_3}) x_i x_{u_2}x_{u_3}x_{u_4} P_{T_k^m\setminus \{i,u_2,u_3,u_4\}}(x) \rp|\\
\leq \sum_{x \in \{-1,1\}^n} \frac{\epsilon}{n^4} \sum_{u_2 \in \cup_{j \leq m} U_j, u_3 \in U_{m+1}, u_4 \in \cup_{j \geq m+2}U_j}
\sum_{x \in \{-1,1\}^n}
 |P_{T_k^m\setminus \{i,u_2,u_3,u_4\}}(x)|
\end{align*}
Now, as we explained, $P_{T_k^p\setminus \{i,u_2,u_3,u_4\}}$ is not a true probability distribution, hence we cannot get rid of the absolute values. 
However, we do have some information about the expression of $P_{T_k^m\setminus \{i,u_2,u_3,u_4\}}$. Indeed, it is generated by a tree like $T_k^m$ with the quartet $i,u_2,u_3,u_4$ removed. This breaks $T_k^m$ into disconnected subtrees, but the expression on each subtree is still not a probability distribution. However, we can do the following: reverse the cut-paste process in each component separately, using the exact same order. Then, you end up with a true distribution, not the original one, but still one that is defined on the disconnected tree topology. Moreover, the number of quartets that are displaced using this process is less than the number that was 
displaced using the original process until time $k,m$. Hence, we can use the inductive hypothesis to prove
$$
 \sum_{x \in \{-1,1\}^n} |f_x^{T_k^{m+1}}(\alpha) - f_x^{T_k^m}(\alpha)|  \leq \frac{\epsilon r_{km}}{n^4} (1 + \frac{\epsilon}{n^4} K'_{ij}) \leq 2 \frac{r_{km}\epsilon}{n^4}
$$
where we use $K'_{ij}$ to denote the number of misplaced quartets in the tree with the disconnected components and $r_{km}$ is the number of misplaced quartets in the current step from $T_k^m \to T_k^{m+1}$. Finally, using Equation \eqref{eq:Kij} we conclude that
$$
\sum_{x \in \{-1,1\}^n} |f_x^T(\alpha) - f_x^{T_i^j}(\alpha)|  \leq 2\frac{\epsilon}{n^4} (\sum_{k<i, m\leq l_k} r_{km} + \sum_{m \leq j} r_{im}) = 2\frac{\epsilon K_{ij}}{n^4}
$$
Hence, the inductive step is complete. 
Applying this result for $T_n^{l_n}$ we get the result of the Theorem. 







\end{proof}


